Bridging Unsupervised and Supervised Depth from Focus via All-in-Focus Supervision

Depth estimation is a long-lasting yet important task in computer vision. Most of the previous works try to estimate depth from input images and assume images are all-in-focus (AiF), which is less common in real-world applications. On the other hand, a few works take defocus blur into account and consider it as another cue for depth estimation. In this paper, we propose a method to estimate not only a depth map but an AiF image from a set of images with different focus positions (known as a focal stack). We design a shared architecture to exploit the relationship between depth and AiF estimation. As a result, the proposed method can be trained either supervisedly with ground truth depth, or \emph{unsupervisedly} with AiF images as supervisory signals. We show in various experiments that our method outperforms the state-of-the-art methods both quantitatively and qualitatively, and also has higher efficiency in inference time.

==> 5_limitation.tex <==
\section{Limitations}
\yulunliu{Show a failure case of dynamic scene while other methods also fail.}
\albert{Do we need to train the CVPR method with the recurrent modelt?}
\begin{figure}[]
    \centering
    \renewcommand{\tabcolsep}{2pt} %
    \renewcommand{\arraystretch}{2} %
    \newcommand{\imagewidth}{0.38\columnwidth}
    \resizebox{\linewidth}{!}{%
    \begin{tabular}{cccc}
        & Zero Motion & Small Motion & Large Motion \\
        \raisebox{3\normalbaselineskip}[0pt][0pt]{
            \rotatebox[origin=c]{90}{Pred AiF}} &
            \includegraphics[width=\imagewidth]{fig/Baseline/Mobile_Phone_Dataset/Ours_flyingthings3d/AiF/zeromotion.jpg} &
            \includegraphics[width=\imagewidth]{fig/Baseline/Mobile_Phone_Dataset/Ours_flyingthings3d/AiF/smallmotion.jpg} &
            \includegraphics[width=\imagewidth]{fig/Baseline/Mobile_Phone_Dataset/Ours_flyingthings3d/AiF/largemotion.jpg} \\
        \raisebox{3\normalbaselineskip}[0pt][0pt]{
            \rotatebox[origin=c]{90}{After Calib}} &
            \includegraphics[width=\imagewidth]{fig/Baseline/Mobile_Phone_Dataset/Ours_flyingthings3d/depth/zeromotion.jpg} &
            \includegraphics[width=\imagewidth]{fig/Baseline/Mobile_Phone_Dataset/Ours_flyingthings3d/depth/smallmotion.jpg} &
            \includegraphics[width=\imagewidth]{fig/Baseline/Mobile_Phone_Dataset/Ours_flyingthings3d/depth/largemotion.jpg} \\
        \raisebox{3\normalbaselineskip}[0pt][0pt]{
            \rotatebox[origin=c]{90}{Before Calib}} &
            \includegraphics[width=\imagewidth]{fig/Baseline/Mobile_Phone_Dataset/Ours_flyingthings3d/depth_original/zeromotion.jpg} &
            \includegraphics[width=\imagewidth]{fig/Baseline/Mobile_Phone_Dataset/Ours_flyingthings3d/depth_original/smallmotion.jpg} &
            \includegraphics[width=\imagewidth]{fig/Baseline/Mobile_Phone_Dataset/Ours_flyingthings3d/depth_original/largemotion.jpg} \\
    \end{tabular}%
    }
    \caption{Limitations on camera motion. Mobile Phone Dataset with Motion}
    \label{fig:limitation}
\end{figure}

